Towards High-Fidelity Synthetic Multi-platform Social Media Datasets via Large Language Models

Social media datasets are essential for research on a variety of topics, such as disinformation, influence operations, hate speech detection, or influencer marketing practices. However, access to social media datasets is often constrained due to costs and platform restrictions. Acquiring datasets that span multiple platforms, which is crucial for understanding the digital ecosystem, is particularly challenging. This paper explores the potential of large language models to create lexically and semantically relevant social media datasets across multiple platforms, aiming to match the quality of real data. We propose multi-platform topic-based prompting and employ various language models to generate synthetic data from two real datasets, each consisting of posts from three different social media platforms. We assess the lexical and semantic properties of the synthetic data and compare them with those of the real data. Our empirical findings show that using large language models to generate synthetic multi-platform social media data is promising, different language models perform differently in terms of fidelity, and a post-processing approach might be needed for generating high-fidelity synthetic datasets for research. In addition to the empirical evaluation of three state of the art large language models, our contributions include new fidelity metrics specific to multi-platform social media datasets.

==> sections/evaluations.tex <==
\section{Evaluation of Synthetic Social Media Posts}
\label{sec:results}
%Recall that we have two real multi-platform datasets. An elections dataset which contains posts made by common Twitter, Facebook, and Reddit users, and an influencers dataset which contains posts made by popular users on Instagram, TikTok, and YouTube. 
We evaluate the textual fidelity of the synthetic posts compared to real posts.
We measure fidelity along four dimensions. 
First, we compare the occurrence of platform-specific textual features typical to social media posts, namely hashtags, user tags, URLs, and emojis.
Second, we compare the sentiment of synthetic to real posts. 
Third, we assess the diversity and coherence of topics found in synthetic posts compared to real posts.
And finally, we measure text similarity between real and synthetic posts in the embedding space.

\subsection{Hashtags, User Tags, URLs and Emojis in Synthetic Data}

Table~\ref{tab:occurentokens} presents the average number of hashtags, user tags, URLs, and emojis, respectively, per real and synthetic post, along with distinct occurrences of these tokens. 
On average, chatGPT tends to create more hashtags for Twitter, Facebook, YouTube and even Reddit, where the use of hashtags in reality is rather low. 
However, hashtags are underrepresented in the synthetic data for Instagram and TikTok, whereas in our Dutch influencers dataset hashtags are heavily used for monetization. 
In terms of hashtag diversity, we observe a larger number of distinct hashtags in the synthetic data than in the real (shown between parentheses in Table~\ref{tab:occurentokens}), indicating lower hashtag reuse among posts in the synthetic datasets than in reality.  
On social media platforms, hashtags are meant to connect posts with similar topics, yet,  understandably, chatGPT misses this point. 
This difference was also observed in~\cite{bertaglia2024instasynth} and likely relates to the sequential manner in which LLMs work, without trying to make connections between individual outputs. 
However, this may also suggest that prompting strategies that emphasize shared hashtags among the examples given in prompts could lead to more realistic generated datasets.


\begin{table}[!h]
\caption{The average number of lexical features per message in the real and synthetic social media datasets. The number of distinct tokens appears within parentheses. Each data collection includes 1000 social media posts from each platform.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llrrrrrrr@{}}

\toprule
\textbf{Platform} & \textbf{Token} & \textbf{Real} & \multicolumn{3}{c}{\textbf{Platform Agnostic}} & \multicolumn{3}{c}{\textbf{Platform Aware}} \\ \cmidrule(lr){4-6} \cmidrule(lr){7-9}
 &  &  & \textbf{T=0.7 P=1} & \textbf{T=1 P=0.7} & \textbf{T=1 P=1} & \textbf{T=0.7 P=1} & \textbf{T=1 P=0.7} & \textbf{T=1 P=1} \\ \midrule
\multirow{4}{*}{Twitter} & Hashtag & 1.19 (964) & 1.77 (1402) & 1.74 (1403) & 1.84 (1458) & 1.73 (1378) & 1.69 (1304) & 1.81 (1405) \\
 & Tag & 1.02 (930) & 0.72 (680) & 0.70 (654) & 0.56 (516) & 0.65 (608) & 0.60 (555) & 0.54 (510) \\
 & URL & 0.35 (356)& 0.13 (126) & 0.12 (123) & 0.07 (75) & 0.06 (62) & 0.07 (69) & 0.05 (50) \\
 & Emoji & 0.30(175) & 0.34 (183) & 0.32 (186) & 0.43 (225) & 0.31 (163) & 0.26 (143) & 0.37 (193) \\ \midrule
\multirow{4}{*}{Facebook} & Hashtag & 0.92 (830) & 1.74 (1420) & 1.78 (1420) & 1.75 (1381) & 1.28 (1080) & 1.35 (1114) & 1.38 (1118) \\
 & Tag & 0.05 (48) & 0.01 (16) & 0.19 (22) & 0.03 (36) & 0.01 (16) & 0.02 (19) & 0.01 (9) \\
 & URL & 0.17 (190) & 0.04 (44) & 0.05 (56) & 0.04 (38) & 0.04 (39) & 0.04 (44) & 0.03 (32)\\
 & Emoji & 0.00 (3) & 0.10 (78) & 0.08 (55) & 0.15 (99) & 0.11 (22) & 0.07 (58) & 0.17 (95) \\ \midrule
\multirow{4}{*}{Reddit} & Hashtag & 0.14 (72) & 1.24 (963) & 1.15 (830) & 1.15 (908) & 0.13 (118) & 0.10 (94) & 0.12 (128) \\
 & Tag & 0.00 (2) & 0.00 (2) & 0.00 (1) & 0.03 (4) & 0.00 (1) & 0.00 (1) & 0.00 (1) \\
 & URL & 0.09 (110) & 0.01 (11) & 0.01 (16) & 0.01 (14) & 0.01 (14) & 0.02 (19) & 0.01 (14) \\
 & Emoji & 0.01 (3) & 0.08 (45) & 0.04 (31) & 0.11 (63) & 0.02 (22) & 0.01 (14) & 0.02 (16) \\  \midrule
 \hline
\multirow{4}{*}{Instagram} & Hashtag & 3.64 (2058) & 2.34 (1835) & 2.39 (1874)& 2.20 (1763) & 2.65 (2115) & 2.69 (2133) & 2.51 (2122) \\
 & Tag & 0.77 (539) & 0.26 (250) & 0.27 (254) & 0.26 (245) & 0.28 (272) & 0.27 (260) & 0.29 (274) \\
 & URL & 0.01 (8) & 0.00 (2) & 0.00 (2) & 0.00 (2) & 0.00 (1) & 0.00 (1) & 0.00 (1) \\
 & Emoji & 1.40 (576) & 1.64 (558) & 1.62 (527) & 1.63 (553) & 1.90 (585) & 1.92 (556) & 1.98 (563) \\ \midrule
\multirow{4}{*}{TikTok} & Hashtag & 3.41 (1805) & 2.80 (1964) & 2.76 (1909) & 2.77 (2031) & 3.16 (2069) & 3.19 (2086) & 3.21 (2166) \\
 & Tag & 0.20 (173) & 0.10 (95) & 0.10 (98) & 0.10 (99) & 0.10 (97) & 0.11 (107) & 0.12 (113) \\
 & URL & 0.00 (0) & 0.00 (0) & 0.00 (0) & 0.00 (0) & 0.00 (0) & 0.00 (0) & 0.00 (0) \\
 & Emoji & 1.00 (402) & 1.56 (525) & 1.66 (539) & 1.72 (561) & 1.72 (545) & 1.70 (528) & 1.76 (553) \\ \midrule
\multirow{4}{*}{YouTube} & Hashtag & 1.02 (499) & 2.25 (1291) & 2.28 (1296) & 2.15 (1334) & 2.02 (1245) & 2.06 (1263) & 1.96 (1211) \\
 & Tag & 1.00 (82) & 0.05 (52) & 0.05 (46) & 0.05 (46) & 0.04 (41) & 0.05 (52) & 0.04 (41) \\
 & URL & 8.67 (2489) & 0.34 (229) & 0.37 (257) & 0.40 (288) & 0.98 (613) & 1.11 (726) & 0.96 (589)  \\
 & Emoji & 1.67(141) & 0.91 (297) & 0.78 (285) & 0.95 (334) & 1.56 (435) & 1.31 (420) & 1.55 (432) \\ \bottomrule
\end{tabular}%
}

\label{tab:occurentokens}
\end{table}
%(higher use compared to content-aware and increasing both parameters also increases these features. The trend in the frequency of features for synthetic Facebook and Reddit data significantly differs from what was observed in the Twitter data. 
Tagging other platform users is common on Twitter, Instagram and YouTube and almost non-existent on Reddit. 
In our experiments, chatGPT underestimates the use of user tags in all cases, except for Reddit, where it correctly estimates virtually no use of such tags. 
The same pattern of no tag reuse is evident. 
For example, in the case of YouTube influencers, where on average every post out of the 1000 in our dataset tags one out of 82 distinct users, in synthetic posts each tagged user is distinct from the users tagged in other posts. 
This time, due to generating fewer user tags on average per post, chatGPT also generates fewer unique such tags than there are in our datasets. 

The number of URLs included in posts is also underrepresented in synthetic data, most notably for YouTube, where influencers typically include their accounts on other platforms via web addresses. 
However, due to the relatively low number of URLs present in both datasets (except the YouTube video descriptions), the difference between real data and synthetic data in this metric is limited. 

Finally, emojis are accurately represented in the synthetic datasets for most platforms overall.
Remarkably, there is a clear distinction between the platforms represented by our two datasets: the Dutch influencers use many emojis, while in the US election conversations there are significantly fewer. 
While unclear if the topics or the platform practices are determining this difference, it is notable that chatGPT accurately captures this difference. 
Again, synthetically generated posts include a much larger variety of emojis than in our real data, especially for the more restrained platforms, such as Facebook and Reddit. 

While we experimented with two prompting strategies and three combinations of parameters each, we could not see a consistent benefit of any one combination in these lexical metrics. 
%Platform-aware prompting tends to perform closer to the real data for YouTube and Reddit than the platform-agnostic prompt. 


\subsection{Sentiment Analysis} 
Moving beyond lexical tokens, we compare sentiments expressed in generated content with real data. 
%Sentiment analysis is a relevant task for evaluating the fidelity of synthetic social media data because it captures the emotional tone that characterizes communication across different platforms. We use sentiment distributions as a fidelity metric, specifically by measuring and comparing the sentiments expressed in synthetic datasets against those in real datasets. 
We employed the \emph{cardiffnlp/twitter-roBERTA-base-sentiment-latest} model proposed by Loureiro et al.~\cite{loureiro-etal-2022-timelms} available at Hugging Face\footnote{https://huggingface.co/cardiffnlp/twitter-roberta-base-sentiment-latest} to classify posts as \textit{positive}, \textit{negative}, or \textit{neutral}.
The model is based on the RoBERTa architecture~\cite{Liu2019RoBERTaAR} and is pre-trained for language modelling on ~124M tweets and then fine-tuned for sentiment analysis on the TweetEval benchmark~\cite{barbieri2020tweeteval}.
Table~\ref{tab:sent_inf_ds} presents the percentage of posts belonging to a particular sentiment category for each platform.
We observe that generated content is more positive and less negative than reality for all platforms.
Neutral sentiment is also under-expressed in synthetic content across all platforms except for Reddit.
Recent work~\cite{das2024offlandat, dutta2023down, hartvigsen2022toxigen,zhang2023comprehensive} has shown the use of LLMs for generating toxic content. 
Therefore, our observed outputs from the chatGPT suggest that efforts are being made to decrease negativity in the generated content.
However, from the standpoint of improving fidelity, prompting techniques that use positive intent as presented in~\cite{das2024offlandat} could generate content that better matches the negative sentiment in real posts.

Again, the prompting strategy and the parameters used do not yield any consistent lessons. 
The relative tone of the two datasets is maintained for all settings: the synthetic US election posts are classified as more negative than the synthetic posts generated from the Dutch influencers examples, which accurately reflects the real datasets, independent of prompting and GPT parameters.
In the rest of our evaluation section we will only include the default parameters (temperature $T=1$, probabilistic sampling $P=1$) for the two prompting strategies.  

\begin{table}[H]
\caption{Percentage of posts out of a collection of 1000 for each platform and setting that are classified based on sentiment analysis.}
\begin{tabular}{@{}llrrrrrrr@{}}
\toprule
\textbf{Platform} & \textbf{Sentiment} & \textbf{Real} & \multicolumn{3}{c}{\textbf{Platform Agnostic}} & \multicolumn{3}{c}{\textbf{Platform Aware}} \\ \cmidrule(lr){4-6} \cmidrule(lr){7-9}
 &  &  & \textbf{T=0.7 P=1} & \textbf{T=1 P=0.7} & \textbf{T=1 P=1} & \textbf{T=0.7 P=1} & \textbf{T=1 P=0.7} & \textbf{T=1 P=1} \\ 
 \hline
Twitter & Negative & 46.76 & 32.87 & 33.30  & 26.75 & 31.86 & 31.85 & 29.50 \\              
    & Neutral  & 21.06  & 17.93  & 15.91  & 15.50     & 15.48   & 16.37   & 13.50  \\
    & Positive                      & 32.18                       & 49.20                                                                            & 50.79                                                                             & 57.75                                                                         & 52.66                                                                                 & 51.78                                                                                 & 57.00                                                                               \\ 
                      
                         \hline
                                      & Negative                      & 34.19                       & 22.74                                                                            & 24.44                                                                             & 19.77                                                                         & 21.98                                                                                 & 23.47                                                                                 & 18.97                                                                               \\
Facebook                              & Neutral                       & 31.80                       & 29.73                                                                            & 29.77                                                                             & 27.28                                                                         & 26.57                                                                                 & 26.95                                                                                 & 27.51                                                                               \\
                                      & Positive                      & 34.01                       & 47.53                                                                            & 45.79                                                                             & 52.95                                                                         & 51.45                                                                                 & 49.58                                                                                 & 53.52                                                                               \\ \hline 
                                      & Negative                      & 81.91                       & 57.54                                                                            & 56.54                                                                             & 56.03                                                                         & 65.10                                                                                 & 62.93                                                                                 & 60.95                                                                               \\
Reddit                                & Neutral                       & 7.95                        & 15.25                                                                            & 15.94                                                                             & 14.56                                                                         & 15.29                                                                                 & 17.45                                                                                 & 18.43                                                                               \\
                                      & Positive                      & 10.14                       & 27.21                                                                            & 27.52                                                                             & 29.41                                                                         & 19.61                                                                                 & 19.62                                                                                 & 20.62                                                                               \\ \hline \midrule
                                      & Negative                      & 3.3                       & 1.9                                                                            & 2.0                                                                             & 1.3                                                                         & 0.9                                                                                 & 0.6                                                                                 & 0.7                                                                               \\

Instagram                 & Neutral                    & 29.2                                        & 4.7                              & 5.4                              & 4.7                            & 4.3                              & 5.0                                & 4.6                            \\
                          & Positive                   & 67.5                                        & 93.4                             & 92.6                             & 94.0                           & 94.8                             & 94.4                             & 94.7                           \\ \hline
                          & Negative                   & 7.1                                         & 4.6                              & 4.7                              & 5.1                            & 6.2                              & 7.1                              & 5.8                            \\
TikTok                    & Neutral                    & 39.0                                        & 9.4                              & 9.5                              & 10.8                           & 14.4                             & 15.8                             & 14.7                           \\
                          & Positive                   & 53.9                                        & 86.0                             & 85.5                             & 84.1                           & 79.4                             & 77.1                             & 79.5                           \\ \hline
                          & Negative                   & 2.0                                         & 1.0                              & 0.1                              & 1.1                            & 1.0                              & 0.7                              & 0.7                            \\
YouTube                   & Neutral                    & 40.0                                        & 8.3                              & 8.7                              & 6.3                            & 8.0                              & 8.9                              & 7.0                            \\
                          & Positive                   & 58.0                                        & 90.7                             & 90.6                             & 92.6                           & 91.0                             & 90.4                             & 92.3                           \\ \hline
\end{tabular}
\label{tab:sent_inf_ds}
\end{table}

\subsection{Topic Generation and Overlap}
Considering that social media posting behavior revolves around topics, we analyze topics in the synthetic data and compare them with topics in real posts. 
Intuitively, the generated data should be representative of the midterm US 2022 elections and respectively the themes that influencers choose to talk about, yet new topics in these general subjects are welcome for diversity and potential utility of synthetic data.
%The presence of common topics across synthetic and real datasets are a measure of fidelity. 
%In contrast, the presence of new topics in generated datasets highlight the creative ability of LLMs to generate content provided they are related to US elections and influencer-specific topics. 

For topic extraction we used BERTopic~\cite{grootendorst2022bertopic} which is being increasingly used for social media data~\cite{verbeij2024happiness,hanley2023happenstance,hua2022using}.
%BERTopic works in three steps, it first creates sentence embedding vectors for input posts, follows up with clustering of these sentence vectors and finally performs topic representation.
For sentence embedding required by BERTopic, we used all-MiniLM-L6-v2\footnote{https://huggingface.co/sentence-transformers/all-MiniLM-L6-v2}~\cite{wang2020minilm} sentence transformer that works with sentences as well as short paragraphs, which is useful in our case because of the length variety from long Reddit and YouTube posts to short tweets.
%pre-trained on 1B sentence pairs dataset.
We performed minimal text cleaning for optimization purposes. 
Salient features such as hashtags and emojis were abundant in the influencer dataset, and omitting them resulted in posts losing their meanings. 
Therefore, only URLs and stop words were removed during this process.
We focused only on the topics that appeared in at least 10 social media posts on the corresponding platform.
Figure~\ref{fig:inf_ele_real_syn} shows the number of shared and disjoint topics across different platforms in real and synthetic datasets. 
For topic overlap, we applied Open AI's embedding model~\cite{neelakantan2022text} (text-embedding-3-large) on top-10 most representative words for each topic and used cosine similarity for topic comparison with a threshold obtained empirically.

%%We observe that \ainote{the number of platform-specific topics (that do not appear in the most popular topics on the other platforms) tends to decrease in synthetic datasets compared to the original data. The size of the intersection, however, remains remarkably similar. TBC}.

\begin{figure}[!htb]
\centering
\begin{subfigure}{0.16\textwidth}
%    \centering
\includegraphics[width=1.3\linewidth,trim={5cm 1.8cm 1.3cm 0},clip]{images/Election_Real_Dataset.png}
    \caption{Real (US)}
\end{subfigure}
\begin{subfigure}{0.16\textwidth}
%    \centering
\includegraphics[width=1.3\linewidth,trim={5cm 1.8cm 1.3cm 0},clip]{images/Election_Synthetic_Platform_Agnostic.png}
    \caption{Agnostic (US)}
\end{subfigure}
\begin{subfigure}{0.16\textwidth}
%    \centering
\includegraphics[width=1.3\linewidth,trim={5cm 1.8cm 1.3cm 0},clip]{images/Election_Synthetic_Platform_Aware.png}
    \caption{Aware (US)}
\end{subfigure}
\begin{subfigure}{0.16\textwidth}
%    \centering
\includegraphics[width=1.3\linewidth,trim={4.8cm 1.8cm 1.1cm 0},clip]{images/Influencer_Real_Dataset.png}
    \caption{Real (NL)}
\end{subfigure}
\begin{subfigure}{0.16\textwidth}
%    \centering
\includegraphics[width=1.3\linewidth,trim={4.8cm 1.8cm 1.1cm 0},clip]{images/Influencer_Synthetic_Platform_Agnostic.png}
    \caption{Agnostic (NL)}
\end{subfigure}
\begin{subfigure}{0.16\textwidth}
%    \centering
\includegraphics[width=1.3\linewidth,trim={4.8cm 1.8cm 1.1cm 0},clip]{images/Influencer_Synthetic_Platform_Aware.png}
    \caption{Aware (NL)}
\end{subfigure}
\caption{Topic overlap among platforms in the real and synthetic datasets. Platform-agnostic/aware prompts, $P=1$, $T=1$.}
\label{fig:inf_ele_real_syn}
\end{figure}



%Because hashtags were not removed to keep all the semantic meaning, some topic words couldn't be vectorized properly, even with state-of-the-art models like the one we used. To mitigate that \hnote{we fine-tuned the similarity threshold to find similarity and retain granularity at the same time. After several modifications, we decided on a threshold of 0.48}. 
%\hnote{for demonstration we used platform agnostic scenario with default parameters and compared it with real data (I don't know how else I can say this)}
%figures Below show topic overlap between platforms in real and synthetic datasets:


%Table~\ref{tab:inf_ele_topics} presents representative names of topics (generated through GPT4 prompting) common across all (or any two) platforms for influencers and elections datasets.

%We consider synthetic data generated through platform-agnostic prompting in this section.
In the elections dataset of real posts, there is more topic diversity on Facebook and Reddit than on Twitter. 
Both prompting approaches can replicate the topic diversity, though not as much in the case of Facebook. Platform-aware prompts generate more topics in Reddit, perhaps because Reddit post lengths are the highest among all platforms, giving chatGPT more grounding. 
The topic `Voter Engagement' appears common in all platforms, both in real and synthetic (platform agnostic) data.
`Women Reproduction Rights' appears as a common topic across Facebook and Reddit. 
Platform agnostic prompting generates four topics of which two (`Mail-in Voting' and `Women Reproduction Rights') are the same as those present in the real posts.
In the influencer dataset of real posts, we observe that topics related to health, wellness, and fitness occur across all platforms. 

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.75\linewidth]{images/Election_Word_Cloud_Platform_Agnostic.png}
    \caption{Topic overlap between real and synthetic (platform agnostic) data on the US elections~(a). Word clouds of unique topics in the real dataset~(b), common topics~(c), and new topics in the synthetic data~(d) on US elections.}
    \label{fig:EDC_plt_ag}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.75\linewidth]{images/Influencer_Word_Cloud_Platform_Aware.png}
    \caption{Topic overlap between real and synthetic (platform aware) data on the Dutch influencers~(a). Word clouds of unique topics in the real dataset~(b), common topics~(c), and new topics in the synthetic data~(d) on Dutch influencers.}
    \label{fig:IDC_plt_aw}
\end{figure}







\iffalse
Compared to the real datasets, both prompting strategies resulted in more topics across all platforms. The only exception to this trend is Twitter, where the number of topics did not change significantly. One reason for this odd behaviour is the shorter average text length in Twitter posts, which makes it harder for the topic model to extract from it. YouTube and TikTok showed the most deviation, which can be attributed to the excessive use of diverse hashtags in their posts and YouTube captions containing several different promotions within a single post. \hnote {Maybe this is the reason for almost doubling the number of topics for YouTube and TikTok in every scenario}Across prompting strategies, platform-aware resulted in a higher number of topics compared to the platform-agnostic approach, and reducing the values of both parameters resulted in a higher number of topic variations. Facebook demonstrated an exception in this trend where higher values of both parameters resulted in lower diversity in the generated topics in both strategies. 




\begin{table}[!htb]
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
\multirow{2}{*}{Platform} & \multicolumn{1}{l}{\multirow{2}{*}{Real}} & \multicolumn{3}{c}{Platform Agnostic}  & \multicolumn{3}{c}{Platform aware} \\
& \multicolumn{1}{l}{}& \multicolumn{1}{l}{T= 0.7,   P= 1} & \multicolumn{1}{l}{T= 1, P= 0.7} & \multicolumn{1}{l}{T= 1, P= 1} & \multicolumn{1}{l}{T= 0.7, P= 1} & \multicolumn{1}{l}{T= 1, P= 0.7} & \multicolumn{1}{l}{T= 1, P= 1} \\ 
\midrule
Instagram & 11  & 9  & 8   & 10                             & 8                                & 16                               & 15                             \\
TikTok                    & 8                                           & 7                                  & 12                               & 9                              & 18                               & 18                               & 16                             \\
YouTube                   & 10                                          & 19                                 & 18                               & 27& 23                               & 22                               & 25\\
Facebook                  & 21                                          & 16                                 & 19                               & 14                             & 20                               & 10                               & 8                              \\
Twitter                   & 3                                           & 3                                  & 3                                & 2                              & 2                                & 2                                & 2                              \\
Reddit                    & 14                                          & 19                                 & 26                               & 15                             & 16                               & 14                               & 18                             \\ \bottomrule
\end{tabular}
\caption{Comparison of counts of extracted topics for both prompting strategies and their parameters across the platforms.\rnote{redundant table, will remove in final pass.}}
\label{tab:res_topic_counts}
\end{table}
\fi

Figures~\ref{fig:EDC_plt_ag},~\ref{fig:EDC_plt_aw},~\ref{fig:IDC_plt_ag}, and ~\ref{fig:IDC_plt_aw} present topic overlap between real and synthetic (both prompting) datasets along with word clouds of topic unique and common across datasets.
There are fewer topics in generated content in elections. 
In contrast, for the influencers data, generated content has more topics.
The word clouds are produced from the text generated by GPT 4 as descriptions of the top 10 words that describe a topic extracted with Bert. 
We observe that discussions in the synthetic data remain on the same general subjects as in the real datasets: for example, the synthetic US election datasets include state names (e.g., Arizona, Florida), typical election terminology (candidate, vote, ballot, absentee), politicians active in this context (Stefanik, Desantis, Feterman, Biden), and timely topics (border security, the opioid crisis, the release of Brittney Griner). 
Different topics and keywords have become more popular in the synthetic dataset, thus appearing in the word cloud: for example, ``Arabia'' in the word cloud representing topics unique to the synthetic data in Figure~\ref{fig:EDC_plt_ag} appears in the original dataset (in the context of oil prices) but it is emphasized significantly in the generated data.

In comparison, we observe more overlapping topics between platforms in the synthetic dataset of influencers.
Physiotherapy appears in synthetic data generated from both prompts on Instagram and YouTube. 
Amusement and games-related topics appear across all datasets in TikTok and YouTube.
In general, both synthetic influencers datasets stay on subjects specific to influencers' monetization practices, such as skin care, diets, life style (e.g., baking, chilling). 

%across platforms, indicating good generation capabilities but also recurring topics across platforms. 
%Further, we observe that topics within Instagram and TikTok are more in the real dataset, as compared to the platform agnostic prompt generated data.
%In contrast, the synthetic dataset for YouTube generated far more number of topics as compared to the real data due to large size of video descriptions.


%Overall, we find that synthetic datasets have more shared topics than real ones}. Another way that we can compare topic overlap is to compare real datasets with their synthetic counterparts. For this, we take the union of the topics between platforms $[A \cup B \cup C]$ to ensure topic uniqueness. The figures below show the result for this comparison:
%\hnote{ in \ref{fig:EDC} we see that there are fewer unique topics in synthetic datasets compared to the real one. This can be partly explained by more shared topics in synthetic data and topic modeling limitations. (Maybe adding the data from the average token count and showing that the average length of posts is halved can explain this more. Topic extraction models discover fewer topics in shorter texts.)
%This pattern is reversed in \ref{fig:IDC}. Despite there being more shared topics in the synthetic than in the real dataset, the high topic count from YouTube which was explained before, compensates and overcomes this.}

\subsection{Embedding Similarity}
Most downstream tasks are solved by converting text into embedding vectors. Therefore, assessing the similarity of generated content with real content in embedding space becomes important.
%Embedding Similarity provides another method to assess similarities and differences between the real and synthetic datasets. To accomplish this, the same Embedding Method used in topic similarity was employed
To evaluate the similarity between real and synthetic social media posts, we used OpenAI's \textit{text-embedding-3-large} model~\cite{neelakantan2022text} to convert all text into embedding vectors. We then calculated pairwise cosine similarity for all possible pairs drawn from real and synthetic posts. To measure similarity, we selected the top 1000 highest similarity scores from each set and computed their average. This average represents the central tendency of the most similar pairs, providing a focused measure of similarity that highlights the best matches between the datasets. Additionally, we computed the average of all similarity scores across each dataset to establish a baseline, giving an overall sense of similarity regardless of the top matches. 
Table \ref{tab:res_embedding} displays the similarity matrix for platform agnostic and platform aware prompts with default settings in the election and the influencer dataset. 
In our experiment, platform-agnostic prompts yielded content with slightly higher similarity scores than the platform-aware prompt. Overall, both prompts generate content similar to the real dataset. Among the platforms, Facebook and YouTube exhibited the highest similarity for both prompting strategies, and Reddit and TikTok exhibited the lowest similarity. Our baseline showed that similarity in other cases is low at around 0.24.
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[H]
\begin{tabular}{@{}l{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}cc}
\toprule
\multirow{2}{*}{Platform} & \multicolumn{2}{c}{Platform Agnostic} & \multicolumn{2}{c}{Platform Aware}\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& \multicolumn{1}{c}{Top 1k} & Average& Top 1k&Average\\
\hline
Facebook                  & 0.824&0.234& 0.815&0.235\\
Twitter                   & 0.802&0.229& 0.804&0.233\\
Reddit                    &  0.762& 0.263& 0.754&0.261\\
 Instagran& 0.705& 0.201& 0.695&0.205\\
 TikTok& 0.693& 0.198& 0.682&0.210\\
 YouTube& 0.830& 0.273& 0.875&0.291\\
 \bottomrule
 \end{tabular}
\caption{Similarity matrix computed using cosine distance for Platform Agnostic and Platform Aware Prompt and T= 1, P= 1 parameters for Election and Influencer dataset.}
\label{tab:res_embedding}
\end{table}

\begin{figure}[H]
    \centering

    % Row 1 – US election per platform
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{US_FB_Platform.png}
        \caption{US – Facebook}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{US_Twi_Platform.png}
        \caption{US – Twitter}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{US_Red_Platform.png}
        \caption{US – Reddit}
    \end{subfigure}

    % Row 2 – Dutch influencers per platform
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{Dutch_Ins_Platform.png}
        \caption{Dutch – Instagram}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{Dutch_TT_Platform.png}
        \caption{Dutch – TikTok}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{Dutch_YT_Platform.png}
        \caption{Dutch – YouTube}
    \end{subfigure}

    % Row 3 – Multi-platform
    \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\linewidth]{US_MPTM.png}
        \caption{US – Multi-Platform}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \includegraphics[width=\linewidth]{Dutch_MPTM.png}
        \caption{Dutch – Multi-Platform}
    \end{subfigure}

    \caption{t-SNE visualizations of US and Dutch datasets across different social media platforms.}
    \label{fig:tsne_summary}
\end{figure}
To visualize embedding vectors, we created t-SNE plots using the embeddings of both real and synthetic datasets with the default settings (T=1, P=1). For each 1000 data points across all scenarios (platform aware, platform agnostic, and real), we apply K-means clustering (K=50) and represent cluster centroids as dots in Figure~\ref{fig:t-sne}. %Finally, we reduced the dimensionality of the data to two dimensions using the t-SNE method and generated the plots for visualization.
We experimented with different perplexity values and found consistent results, the plots are drawn on default perplexity value.
While t-SNE has limitations, it presents a good estimate for the preservation of local structure in data. 
In the election dataset, synthetic data shows high similarity with real data for Facebook.
In the case of Reddit and Twitter, synthetic datasets (platform aware and platform agnostic) show similarities along only one of the reduced dimensions. 
Real Reddit posts appear near to their synthetic counterparts, but for Twitter, they are quite far apart.
%the second axis but were separated along the first axis. The space between these synthetic datasets was filled by the real Reddit data, indicating similarities with both synthetic scenarios on this platform. Twitter data resulted in three distinct clusters; the Platform Aware dataset aligned closely with the real data along the second axis but was separated along the first axis. Conversely, the Platform Agnostic dataset was close along the first axis but diverged on the second axis.
In the influencer dataset, we observe high similarity between real and synthetic video descriptions for YouTube.
For Instagram, both platform-aware and platform-agnostic datasets appear similar but quite separated from the real dataset. 
In the case of TikTok, only platform aware is aligned with real in one dimension, and others are quite far apart from each other. 

==> sections/methodology.tex <==
\section{Synthetic Data Generation via chatGPT}
To generate data, we opted for OpenAI's model GPT-3.5-turbo, which is a text completion model capable of retaining context from previous interactions. It is also the most cost-effective\footnote{https://openai.com/pricing} option among OpenAI's model offerings, making it preferable for generating larger datasets. Another factor that influenced our choice of this model is its compact size compared to other options, which helps reduce the carbon footprint of our approach, especially since we are generating large multi-platform datasets. 
\begin{comment} % rejected by Thales
  Being an older model, makes it more stable in term of changes, making it more reproducible compared to the newer versions.   
\end{comment}

%\ainote{@danial, why? Explain here, please.} 
\begin{comment}
    Well this is a tough one if you ask me. There are multiple reasons now. Most of them are based on little to no evedence but just experience. e.g GPT4 is getting even less reproducible then it was 2 months ago. I discovered this in my lab yesterday when I was having a discussion with my supervisor Henry as he's supervising a student using GPT 4 for sumerizing articles. This is due to the way they are managing resources and loads between regions and time zones. So, they discovered the best time to use it, is something around 2AM Asia time. 
\end{comment}


\begin{figure}[ht]
\centering
{\includegraphics[width=0.8\textwidth]{images/arch_diagram.png}}%
\caption{Pipeline of our methodology for generating and evaluating synthetic social media datasets.}
% Link to edit the diagram: https://lucid.app/lucidchart/ebee82f7-9425-4576-b9ec-ad8d98f91476/edit?viewport_l[…]4MUjXso07N&invitationId=inv_85f1b17b-3e19-4377-ac76-67fbd24ca59b
\label{fig:prompt_struct}
\end{figure}



\noindent 
%\textbf{Prompt Engineering}: 
%We aim to generate multi-platform social media posts for the two datasets, one related to the US elections and the other related to influencers.
We employed various strategies to generate text resembling realistic social media posts.
We began with a basic zero-shot prompt instructing the generation of a specific social media post such as, ``\textit{Generate a Twitter post based on US elections 2022}'', but it proved ineffective in producing diverse results: Upon receiving multiple iterations of the same prompt, chatGPT starts reproducing the same outputs with only minor variations such as adding an emoji or using a different hashtag at the end.
As a consequence, we tried few-shot prompting by providing a variety of contextual examples in prompts.
We experimented with prompts ranging from two to five input examples. 
Generally, using more examples enhanced the diversity and variation in the output, which seemed particularly effective for platforms with shorter messages, such as Twitter. After experimenting with different numbers of grounding examples, across all the platform, we obtained the best results when providing three randomly chosen posts from our real dataset and prompting chatGPT to generate three output posts. Using more than three examples becomes problematic when dealing with platforms like Reddit, where the long text messages are challenging for the token limit of a single API call and for keeping track of context. 

Figure~\ref{fig:prompt_struct} depicts the pipeline of our prompt approach.
We implemented our prompting approach using the OpenAI API\footnote{https://platform.openai.com/docs/introduction}. 
%A role was assigned to the model based on our prompting strategy.
Each prompt specified a desired JSON output format to facilitate the extraction of the generated posts.
\begin{comment}
\rnote{what is temporal info, not clear to me} and their temporal information. 
\end{comment}
Outputs that deviated from the specified JSON format were discarded, as the model occasionally produced invalid results. 
During our initial prompt experience, we observed that chatGPT often ignored the context of the three input examples provided. 
Therefore, we refined the prompt instruction and included phrases like `Using following examples ...', `Based on the examples below ...', and so on. 
This modification improved performance within the given context, aligning results more closely with our real dataset. 
However, after some runs, the chatGPT model often produced results that were mere reproductions of the examples.
Henceforth, we further rephrased our prompt instruction by adding phrases like `generate new posts keeping them true to their content and writing style.'
This prompt instruction encouraged the generation of diverse and novel social media posts, resembling the examples but distinct enough to be considered unique. 
Throughout this process, we observed that the model tended to ignore instructions when the size of the examples was large, likely due to limited attention capacity. To address this issue, we placed a single-line summary of the instructions at the end of the prompt.

%\ainote{so we converged in the end to one way of prompting? Can we include that example here?}

In the end we converged to two distinct types of prompting, referred to as \emph{`platform aware'} and \emph{`platform agnostic'}.
In \emph{platform-aware prompting}, we explicitly ask in the prompt instructions to generate text for the target social media platform. 
This prompting strategy was adopted in the hope of leveraging the model's capability to generate posts with styling characteristics that are typical of the target social media platform.
%The model was informed about the platform by assigning the role of a user on a specific social media platform. Additionally, the main body of the prompt included instructions to generate content for that particular platform. 
In \emph{platform-agnostic prompting}, the chatGPT model was not informed about the target social media platform, but it was asked to keep the generated output similar in content and length to the examples provided.
%by assigning the role of a generic social media user. 
%%In this case, the prompt instruction excluded any reference to any type of social media platform. 
%%This was done in the hope of keeping the model focused on textual content and its length in order to keep the output within the norms of a platform.

\begin{comment}
\textbf{Platform aware}: The model was informed about the platform by assigning the role of a user on a specific social media platform. Additionally, the main body of the prompt included instructions to generate content for that particular platform.
\textbf{Platform agnostic}:The model was kept in dark about the platform by assigning the role of a generic social media user. Furthermore, the main body of the prompt also excluded any mentions of any type of platform, rather the model was instructed to focus on content and its length to keep the output it within the norms of a platform.
\end{comment}

%\noindent \textbf{Model Parameter Tuning}: 
We experimented with different values for the model's two primary parameters, $temperature$ (T) and $top\_p$ (P). % were explored during the generation process. 
$T$ values exceeding 1 yielded highly varied yet extremely artificial results, while those below 0.7 mostly replicated the given examples. 
$T$ values at 0.7 and 1, however, produced realistic variations, which were then selected for further exploration. 
Likewise, the $P$ values exhibited a comparable trend. 
Consequently, values of 1 and 0.7 for both $T$ and $P$ were chosen for further experimentation. 
When both parameters were set to 0.7, sub-optimal results were obtained, and hence this combination was discarded from further experiments.
Eventually, we perform experiments on three combinations of $T$ and $P$ values, namely, <$T$=0.7, $P$=1>, <$T$=1, $P$=0.7>, and <$T$=1, $P$=1>.
%which suggested individual exploration of each parameter. These parameter values were then tested with both prompting strategies across the entire subset designated for generation.

% copied from masters project report here.
\iffalse
\begin{table}[!h]
\caption{Average generation time of each platform depends on the length of their content. \ainote{what do we call tokens here? average tokens per what? (cannot be post, I don't think).}}
    \centering
    \begin{tabular}{c|c|c|c}
         Platform & Twitter & Facebook & Reddit \\
         \hline
         Total Tokens & 32,628 & 101,709 & 113,988\\
         Average Tokens per post & 31.49 & 93.65 & 96.27 \\
         Average Generation Time (mins) & 60 & 90 & 110 \\ 
    \end{tabular}
    
    \label{tab:gen_time}
\end{table}
\fi
% \noindent \textbf{Challenges}: We briefly outlines issues and challenges faced in implementing prompting. 
% First, we observed that the API’s response time varies between 5 to 20 seconds for a single request, making the turnaround time non-deterministic.
% Second, we saw deteriorating quality of outputs in successive API calls.
% Third, for large posts in case of Reddit, we got token exceed errors  occasionally.
% Fourth, chatGPT appeared to ignore instruction when large posted are used for grounding.
\iffalse
\subsection{General Observations} 

While we evaluate the quality of the generated data in the next section, we share some other empirical observations in this section regarding generating larger collections of messages, as per our objective. 

First, we observed that the API’s response time varies between five to 20 seconds for a single request. 
For generating 501 social media posts using 163 API calls, in which each call generates three messages, time varied between 25 and 45 minutes. This time interval depends on the number of tokens in the input, the size of the input post examples, and the number of tokens generated by the model. 
%For the generation of nearly a thousand posts, 1,140 samples were selected from the dataset, resulting in 380 API calls. 
%Table \ref{tab:gen_time} illustrates (\rnote{stats for influencer dataset, if this Table has to remain.}) the average generation time for each platform, with the resulting generation time proportional to the input post length. 
Generating Twitter posts took the least amount of time, averaging 60 minutes, attributed to the smallest content length compared to the other two platforms. Facebook and Reddit generation both required considerably more time, averaging 90 and 110 minutes, respectively. Reddit took more time on average due to its larger content compared to Facebook, on top of which, Reddit also was the only platform that triggered a token overflow limit error during generation.

Second, after making consecutive API calls, we observe that the quality of output deteriorates. 
For instance, when 163 consecutive API requests were executed, one after the other without delay, to generate 501 posts, the output experienced a significant deterioration.
It was consistently observed across all parameter values and prompting strategies, leading to outputs that closely resembled the inputs. 
However, the degradation was resolved when the same set of prompts was used with a two-second delay between consecutive API requests.
%individually, the output showed marked improvement and aligned with the initial experimentation outcomes. To address this issue, a two-second delay was introduced between two API calls, effectively resolving the observed degradation.

Third, social media platforms like Reddit, which feature very large posts, made the chatGPT model generate even larger outputs, which occasionally exceeded the API token limit, causing an overflow error. To address this in the future, we may impose a strict limit on the input and configure the $maxtokens$ parameter to control the output size. 

Fourth, in the case of very large posts, we observe that the model is more prone to ignoring instructions and generating invalid outputs.
This problem was frequently encountered during the generation process, resulting in the loss of some text in the case of larger posts from the generated data. 
A potential solution to this problem in the future could be to move the output format to the end of the prompt with the summarized instructions.

\fi

==> sections/notes.tex <==
\section{Notes}

Focus: extend the accepted/invited HT paper by:
\begin{enumerate}
    \item an additional dataset (Dutch influencers)
    \item additional LLMs (Claude, Google, )
    \item metrics focused on cross-platform datasets
\end{enumerate}

\begin{figure}[htbp]
\centering
\includegraphics[width=10cm]{images/notes-Feb14.jpg}
\end{figure}

Fig. 1.:
%https://lucid.app/lucidchart/407fa310-929f-49bd-bbd9-d2be3cecee45/edit?viewport_loc=189%2C164%2C2230%2C1200%2Cxxo9z1RDCIHH&invitationId=inv_9851ecfe-fb7e-4244-a23e-f3dcdec761d5
%https://lucid.app/lucidchart/407fa310-929f-49bd-bbd9-d2be3cecee45/edit?viewport_loc=-136%2C157%2C3072%2C1653%2Ca3m9FfpFs6~7&invitationId=inv_9851ecfe-fb7e-4244-a23e-f3dcdec761d5


Meeting (7.04):
Discussion among Henry, Rishabh and Anda
\begin{itemize}
    \item Table 1 - to be removed.
    \item Table 2 clarification questions for our better understanding: First three lines, Facebook data doesn’t match Table 1 and likewise for all platforms.
    \item gpt-4o results missing.
    \item sample size for different LLMs in each platform are different; For eg 706 and 903 in FB, are they from the same random process, or generated in two different random process?
\end{itemize}



%The first three lines are our new sampling method using posts of the same topic as the examples, The table generator just so happens to use my internal naming, in hindsight I should've made it clearer what's what, Same with the Positive/Neutral/Negative collumns, that's sentiment and I'll need to label it soon.
%I think some clarification is in order: Litellm was my original name for 4o and can be changed at any time, If necessary I can bump the counts up to 1000 for every single source/LLM and likewise cut-off any messages above 1000 for those that have more samples. Regarding the missmatch between table 1 and the provided new table that may be caused by the fact the newest table uses the entire dataset of the given social media platform instead of 1000 samples. The different result count is a byproduct of incorrectly formatted responses being discarded if they aren't a json or cannot be parsed using the fallback parser, hence some LLMs have a different amount of data as their adherence rates are different. The samples were generated from the same examples, the generation pipeline generates a prompt and then uses it for all the implemented LLMs

% thanks for clarification

%@Nojus: Can we have a meeting tomorrow morning anytime between 9am to 1pm? Only we three: Henry, Rishabh and you. We can have a quick walkthrough of code just for sanity checking (code cleanups can wait, not required right now) and also we can better understand and resolve clarification doubts. I think That'd be possible, how does 9-11 sound?

%yes, works for us.

%great, see you then tomorrow, thanks a lot for quick clarifications. 


Brainstorming with Rishabh on multi-platform comparison metrics (2.04):
\begin{itemize}
    \item represent the data as a bipartite graph (as in the final report), where one class of nodes represent lexical entities (names, hashtags) and the other class of nodes represent platform users who used those entities in their posts. Thus, like in the final report, we will have three different ''colors'' of platform users: say, red, green, blue;
    \item with this representation, we can have ''colored'' degree for the lexical entities (white nodes). We can then compare the synthetic and real datasets represented as above by the absolute difference in color, where the colored degree of a white node is represented by a color in the normalized 0-255 range  as in [r, g, b]. (Thus, we represent for a node A the difference between datasets as [$r_s-r_r$, $g_s-g_r$, $b_s-b_r$]. The intuition is that the closer to white, the closer the synthetic data is to real data on a particular topic.) We only compare the overlapping "white nodes", thus the topics that appear in both synthetic and real datasets. 
    
    \item For the nodes that are not common, we can still represent them as differences in color if we order the nodes by one of their primary colors (say, read). 

    \item number of connected components in the two datasets and the representation of colors per component. 
\end{itemize}


Meeting notes 31.03:

To do by Friday, 4.04: have all numbers updated.
\begin{enumerate}
    \item Nojus: \begin{itemize}
        \item update Tables~\ref{tab:occurentokens} and ~\ref{tab:sent_inf_ds}. Update the captions to reflect what the pics or tables represent.
        \item give Henry the topic vectors and topic-representative words to update fig.~\ref{fig:inf_ele_real_syn}
        \item write a paragraph that lists the models you used for generation and some general something (section~\ref{sec:prompt}). 
        
    \end{itemize}
    \item Henry: 
    \begin{itemize}
        \item check the numbers/examples in Table~\ref{tab:res_embedding}. 
        \item update Fig~\ref{fig:inf_ele_real_syn} on the data from Noah. Update the captions to reflect what the pics or tables represent.
        \item update Figs.~\ref{fig:EDC_plt_ag} and \ref{fig:IDC_plt_aw}, maybe replacing the word counts with something else that makes more sense/it is more telling. Update the captions to reflect what the pics or tables represent. 
        \item update Fig.~\ref{fig:t-sne}. Update the captions to reflect what the pics or tables represent.
    \end{itemize}
\end{enumerate}

\begin{enumerate}
    \item Anda and Rishabh do a writing/editing pass on the paper on the 7.04.
\end{enumerate}


Meeting notes 24.03:
To be done by 31.03 (ideally, with reliable results that we can then write about): 
\begin{itemize}
    \item Thales will try persona-based prompting for the Dutch influencers dataset (create personas based on keyword clusters and specific examples)
    \item Noah will run the topic-based prompting with an LDA model trained on the full datasets. \textbf{We also need to evaluate the topics, maybe before generating the data}
    \item Noah will run Henry's code (prompts from the old paper with the new models) for the Dutch influencers dataset
    
\end{itemize}


Meeting notes 13.03: 
\begin{itemize}


    \item  we need to revise the prompts and decide on them with ack of literature

    \item  do we need to inform the sampling size based on Henry's approach? To answer the question: what sample size from this dataset should we consider? We need to think of this. 

    \item  The objective for the next meeting is to set the parameters and the flow of the paper; to have clear tasks to finish by April 1 with all results; 
    \item we will need to check again the process for the Dutch influencers dataset: do we stay with one language only? do we have the same crossplatform metrics? etc.
\end{itemize}

To do for 24th: 
\begin{enumerate}
    \item schedule a code review session (2--2.5 hours?) <-- Monday, the 24th
    \item (Noah) generate results we can look at (plots, tables, etc.) --> in particular, recreate Tables 1, 2, and 3 (ignore the T and P for now)
    \item Anda and Rishabh: read the paper to see the flow/gaps/etc.
    \item Anda: crossplatform metrics (see Henry's report with the network)
\end{enumerate}



To do (28.02): 
\begin{enumerate}
    \item decide on prompts: 
    \begin{itemize}
        \item persona based: 
        \item topic based: use a combination of posts from all platforms as example to the prompt. 1)~identify popular hashtags/topics across all platforms, say top-k; 2)~select posts which have these popular hashtags; 3)~randomly select n-posts from this filtered posts to be used as examples in prompts. 
    \end{itemize}
\end{enumerate}

Tasks for Noah:
\begin{enumerate}
    \item generate a synthetic dataset using the topic based prompting strategy described above using the US elections real data; 
    \item evaluate this dataset using the very same metrics already in the paper; How do the results compare with what we saw before? 
    \item document your methodology and the results in a separate section (new file in sections folder). 
\end{enumerate}

Task for Henry:
\begin{enumerate}
    \item topic overlap figures
    \item Tsne
    \item embedding similarity rework
    \item topic overlap rework based on Nojus new work on our old data
    \item real vs synthetic for topic overlap for both scenario
\end{enumerate}

\section{New Results (Full Table - backup)}
Results from this table are split across platform traits and sentiment analysis sections.
\begin{table}[htbp]
\centering
\caption{Comparative Analysis of Social Media Content}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llrrrrrrrr}
\toprule
\textbf{Folder} & \textbf{Provider} & \textbf{Positive} & \textbf{Neutral} & \textbf{Negative} & \textbf{Hashtags} & \textbf{Mentions} & \textbf{URLs} & \textbf{Emojis} & \textbf{Total Messages} \\
\midrule
\multirow{3}{*}{LLM Elections (BERT)} & Sampled data & 20.5 & 44.2 & 35.3 & 0.76 & 0.26 & 0.28 & 0.13 & 4500 \\
  & 3.5 Haiku & 28.3 & 23.0 & 48.7 & 1.14 & 0.30 & 0.05 & 0.23 & 1046 \\
  & Gemini 2.0-Flash & 33.7 & 17.6 & 48.7 & 1.77 & 0.18 & 0.04 & 0.05 & 1062 \\
  & GPT-4o & 37.3 & 31.7 & 30.9 & 0.66 & 0.29 & 0.20 & 0.96 & 1070 \\
\midrule
\multirow{3}{*}{LLM Influencer (BERT)} & Sampled data & 43.4 & 52.9 & 3.7 & 2.14 & 0.50 & 3.57 & 2.03 & 4500 \\
  & 3.5 Haiku & 80.5 & 14.6 & 4.9 & 2.45 & 0.80 & 0.63 & 2.83 & 1182 \\
  & Gemini 2.0-Flash & 77.0 & 17.0 & 6.0 & 4.19 & 0.46 & 0.54 & 1.76 & 1138 \\
  & GPT-4o & 89.6 & 8.9 & 1.5 & 1.62 & 0.58 & 0.38 & 6.85 & 1375 \\
\midrule
\multirow{6}{*}{Original Data} & Facebook Data & 25.9 & 58.5 & 15.6 & 0.98 & 0.05 & 0.21 & 0.00 & 1700 \\
  & Instagram Data & 55.7 & 41.9 & 2.4 & 2.65 & 0.56 & 0.03 & 1.95 & 116708 \\
  & Reddit Data & 6.6 & 41.1 & 52.3 & 0.06 & 0.01 & 0.28 & 0.01 & 136308 \\
  & Tiktok Data & 42.5 & 51.6 & 5.9 & 2.88 & 0.29 & 0.00 & 1.28 & 47177 \\
  & Twitter Data & 26.3 & 41.8 & 31.8 & 1.37 & 0.73 & 0.40 & 0.40 & 27629 \\
  & Youtube Data & 30.2 & 68.4 & 1.4 & 0.91 & 0.51 & 11.08 & 2.64 & 128430 \\
\midrule
\multirow{4}{*}{Platform Facebook} & 3.5 Haiku & 51.8 & 34.1 & 14.1 & 1.18 & 0.03 & 0.04 & 0.20 & 1161 \\
  & Gemini 2.0-Flash & 44.4 & 35.9 & 19.7 & 0.99 & 0.02 & 0.05 & 0.00 & 1798 \\
  & GPT-4o & 54.1 & 35.5 & 10.4 & 0.52 & 0.05 & 0.13 & 0.49 & 1486 \\
  & Facebook Data & 29.0 & 53.8 & 17.2 & 0.90 & 0.05 & 0.20 & 0.01 & 4050 \\
\midrule
\multirow{4}{*}{Platform Instagram} & 3.5 Haiku & 77.0 & 21.1 & 1.9 & 0.80 & 0.38 & 0.01 & 1.94 & 1597 \\
  & Gemini 2.0-Flash & 65.2 & 33.0 & 1.8 & 1.91 & 0.42 & 0.02 & 1.31 & 1805 \\
  & GPT-4o & 78.5 & 21.0 & 0.5 & 1.09 & 0.34 & 0.02 & 3.10 & 1795 \\
  & Instagram Data & 56.1 & 41.1 & 2.8 & 2.62 & 0.54 & 0.03 & 1.94 & 4050 \\
\midrule
\multirow{4}{*}{Platform Reddit} & 3.5 Haiku & 10.5 & 25.8 & 63.7 & 0.95 & 0.00 & 0.00 & 0.32 & 1517 \\
  & Gemini 2.0-Flash & 12.1 & 26.4 & 61.5 & 0.51 & 0.00 & 0.02 & 0.01 & 1836 \\
  & GPT-4o & 15.5 & 27.8 & 56.6 & 0.09 & 0.01 & 0.06 & 0.39 & 1686 \\
  & Reddit Data & 6.0 & 42.4 & 51.6 & 0.04 & 0.01 & 0.27 & 0.02 & 4050 \\
\midrule
\multirow{4}{*}{Platform TikTok} & 3.5 Haiku & 55.8 & 38.9 & 5.3 & 1.73 & 0.32 & 0.00 & 1.46 & 1561 \\
  & Gemini 2.0-Flash & 51.2 & 42.5 & 6.2 & 2.66 & 0.23 & 0.00 & 0.99 & 1805 \\
  & GPT-4o & 66.0 & 31.4 & 2.5 & 1.60 & 0.26 & 0.00 & 2.71 & 1765 \\
  & Tiktok Data & 42.4 & 52.0 & 5.7 & 2.84 & 0.30 & 0.00 & 1.29 & 4050 \\
\midrule
\multirow{4}{*}{Platform Twitter} & 3.5 Haiku & 44.1 & 27.2 & 28.7 & 1.32 & 0.57 & 0.09 & 0.37 & 1257 \\
  & Gemini 2.0-Flash & 39.7 & 27.7 & 32.5 & 1.52 & 0.63 & 0.14 & 0.15 & 1804 \\
  & GPT-4o & 51.2 & 28.6 & 20.2 & 0.98 & 0.61 & 0.39 & 1.25 & 1800 \\
  & Twitter Data & 27.0 & 41.4 & 31.6 & 1.41 & 0.72 & 0.41 & 0.39 & 4050 \\
\midrule
\multirow{4}{*}{Platform Youtube} & 3.5 Haiku & 75.4 & 23.1 & 1.5 & 1.22 & 0.39 & 2.21 & 2.44 & 1593 \\
  & Gemini 2.0-Flash & 53.7 & 43.6 & 2.7 & 1.24 & 0.24 & 3.02 & 1.27 & 1833 \\
  & GPT-4o & 65.6 & 33.8 & 0.6 & 0.58 & 0.51 & 1.94 & 6.20 & 1472 \\
  & Youtube Data & 29.1 & 69.6 & 1.3 & 0.93 & 0.51 & 10.82 & 2.57 & 4131 \\
\bottomrule
\end{tabular}
}
\label{tab:main_results}
\end{table}

\input{sections/methodology}

\input{sections/evaluations}

==> sections/what-is-new.tex <==
Our current paper differs from our previous work, titled "Leveraging GPT for the Generation of Multi-Platform Social Media Datasets for Research," published in the Proceedings of the 35th ACM Conference on Hypertext and Social Media, 2024, in the following key aspects:

1. Prompting Technique: We introduce a multi-platform topic-based prompting approach that captures content knowledge across various social media platforms and instructs LLMs accordingly. In contrast, our earlier work utilized example posts from each platform independently to prompt the LLM (GPT-3.5).

2. Model Comparison: This study extends the analysis by implementing our prompting strategy across three popular LLMs, namely, Claude 3.5, Gemini 2.0, and GPT-4o, to compare the quality of generated synthetic posts. The previous study employed only GPT-3.5.

3. Dataset Diversity: We evaluate synthetic social media content generation using two diverse datasets covering six platforms: one centered on U.S. elections and another on influencer posts. Our prior work was limited to the U.S. elections dataset.

4. Fidelity Evaluation: In addition to previous evaluation methods, we incorporate network analysis of named entities mentioned in posts across platforms. This allows us to explore how named entities spread and connect across different social media platforms.

We confirm that we have expanded our paper to adhere to the ACM policy of adding at least 25\% new material. In fact, due to the use of a new dataset and the use of three new LLMs, all our results are new. In addition, we have significant methodological novel contributions that include the topic-aware prompting strategy and the multi-platform-aware fidelity metrics. 
